Streaming Technologies and Serialization Protocols: Empirical Performance Analysis

Efficient data streaming is essential for real-time data analytics, visualization, and machine learning model training, particularly when dealing with high-volume datasets. Various streaming technologies and serialization protocols have been developed to cater to different streaming requirements, each performing differently depending on specific tasks and datasets involved. This variety poses challenges in selecting the most appropriate combination, as encountered during the implementation of streaming system for the MAST fusion device data or SKA's radio astronomy data. To address this challenge, we conducted an empirical study on widely used data streaming technologies and serialization protocols. We also developed an extensible, open-source software framework to benchmark their efficiency across various performance metrics. Our study uncovers significant performance differences and trade-offs between these technologies, providing valuable insights that can guide the selection of optimal streaming and serialization solutions for modern data-intensive applications. Our goal is to equip the scientific community and industry professionals with the knowledge needed to enhance data streaming efficiency for improved data utilization and real-time analysis.

==> sections/appendices.tex <==
\section{\break Name-1}
Appendix goes here

==> sections/biography.tex <==

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/sam.jpg}}]{Samuel Jackson} is a principal data scientist at the UKAEA. He holds a M.Eng degree in software engineering from the University of Aberystwyth. He has previously worked in various roles with the UK's large scale experimental facilities at the Science and Technology Facilities Council. He has been involved in numerous projects towards improving scientific data analysis and reduction workflows. His expertise are in machine learning, software engineering, and high performance computing.
\end{IEEEbiography}

\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/nathan.jpg}}]{Nathan Cummings}  is a Senior Data Engineer at the UKAEA. He holds an MPhys degree in physics from the University of Bath. His interests are data management and the application of the FAIR data principles to fusion data. He works with various members of the international fusion community to drive the development and adoption of standards, as well as using community-developed tools to improve the utility of data for data-intensive applications such as AI/ML pipelines.
\end{IEEEbiography}


\begin{IEEEbiography}[{\includegraphics[width=1in,height=1.25in,clip,keepaspectratio]{figures/authors/saiful.jpeg}}]{Saiful Khan} is a Senior Data Scientist at the STFC. He received his D.Phil. degree in Engineering Science from the University of Oxford, UK where he also conducted post-doctoral research.
He has worked as a data scientist at Horus Security Consultancy and the International Seismological Centre in the UK, and as a software engineer at Oracle and ABB in India.
His research interests include machine learning, data visualization, and software engineering.

\end{IEEEbiography}
